Decay of Coherence and Entanglement of a Superposition State for a Continuous Variable System in an Arbitrary Heat Bath

We consider the case of a pair of particles initially in a superposition state corresponding to a separated pair of wave packets. We calculate \emph{exactly} the time development of this non-Gaussian state due to interaction with an \emph{arbitrary} heat bath. We find that coherence decays continuously, as expected. We then investigate entanglement and find that at a finite time the system becomes separable (not entangled). Thus, we see that entanglement sudden death is also prevalent in continuous variable systems which should raise concern for the designers of entangled systems.

==> figurecaption.tex <==
\begin{figure}
\includegraphics{C_function.eps}
\caption{$C(t)$ versus $\gamma t$ for the single relaxation time $(\tau )$ model at zero temperature, where $\tau =\gamma^{-1}/6$ and $\gamma $ is the Ohmic relaxation time. We note that separability occurs for $\gamma t \gtrsim 6$.}
\end{figure}


